Mixture of Experts Made Intrinsically Interpretable

Neurons in large language models often exhibit \emph{polysemanticity}, simultaneously encoding multiple unrelated concepts and obscuring interpretability. Instead of relying on post-hoc methods, we present \textbf{MoE-X}, a Mixture-of-Experts (MoE) language model designed to be \emph{intrinsically} interpretable. Our approach is motivated by the observation that, in language models, wider networks with sparse activations are more likely to capture interpretable factors. However, directly training such large sparse networks is computationally prohibitive. MoE architectures offer a scalable alternative by activating only a subset of experts for any given input, inherently aligning with interpretability objectives. In MoE-X, we establish this connection by rewriting the MoE layer as an equivalent sparse, large MLP. This approach enables efficient scaling of the hidden size while maintaining sparsity. To further enhance interpretability, we enforce sparse activation within each expert and redesign the routing mechanism to prioritize experts with the highest activation sparsity. These designs ensure that only the most salient features are routed and processed by the experts. We evaluate MoE-X on chess and natural language tasks, showing that it achieves performance comparable to dense models while significantly improving interpretability. MoE-X achieves a perplexity better than GPT-2, with interpretability surpassing even sparse autoencoder (SAE)-based approaches.

==> Sections/intro.tex <==
\section{Introduction}

% Advances in artificial intelligence (AI) have enabled the development of highly capable systems, but their decision-making processes often remain opaque and poorly understood.
% Rapid progress in transformer language modelling ->  poorly understood -> unintended and undesirable outcomes -> interpretability -> Mechanistic interpretability

% A central obstacle to mechanistic interpretability is how to choose a good subsidance of ``features'' as basic unit for interpret. However, the individual neurons of neural network show \textbf{polysemanticity}~\cite{olah2020zoom}, where individual neurons encode multiple, unrelated concepts. This phenomenon complicates efforts to isolate meaningful features in a model's activation space and undermines the ability to attribute specific model behaviors to distinct components. 


% post hoc interp, Sparse dictionary learning techniques, such as Sparse Auto-Encoders (SAEs)~\cite{huben2023sparse}, have been proposed to address this issue by identifying sparse, semantically distinct directions in the activation space. However, these approaches suffer from significant drawbacks: they are computationally expensive~\cite{gao2024scaling,lieberum2024gemma}, require post-hoc analysis, and are not fully faithful since not all features can be recovered after model training. Consequently, these methods are often impractical for large-scale models and provide limited guarantees about the interpretability of the underlying neural network. 


% Transformer-based large language models (LLMs)~\cite{radford2019language,brown2020language,waswani2017attention} have achieved remarkable progress. However, their internal workings remain poorly understood. This gap \bibir{what gap; you did not clarify that. you want to say that this "poorly understood" or "a continuation of it saying "and because of that .. "}often leads to unintended and undesirable outcomes~\cite{hendrycks2023overview,ngo2022alignment}. Addressing these risks \bibir{What risks? you probably want to explicitly mention "risks" in previous sentence. } requires a deeper understanding of how neural networks operate internally, a challenge that lies at the heart of mechanistic interpretability~\cite{elhage2022mechanistic}. \bibir{I feel the sentence above has a few repetition. you said the thing about models being misunderstood twice.}

Transformer-based large language models (LLMs)~\cite{radford2019language,brown2020language,waswani2017attention} have achieved remarkable progress. However, their internal workings remain poorly understood. This lack of understanding often leads to unexpected and potentially harmful behaviors~\cite{hendrycks2023overview,ngo2022alignment}, posing risks in their deployment. To address this, mechanistic interpretability~\cite{elhage2022mechanistic} seeks to uncover how these models process information and reduce potential risks.


% Addressing these risks requires a deeper understanding of how neural networks operate internally, a challenge that lies at the heart of mechanistic interpretability~\cite{elhage2022mechanistic}. \bibir{I feel the sentence above has a few repetition. you said the thing about models being misunderstood twice.}


\begin{figure}
    \centering
    % \includegraphics[width=\linewidth]{Fig/tiser2.pdf}
    \includegraphics[width=\linewidth]{Fig/tiser3.pdf}
    \caption{MoE-X introduces a sparse and wide network architecture designed for interpretability. Compared to dense MLPs, it incorporates both sparsity and a wider structure. Unlike traditional MoE models, it uses sparsity routing based on expert activations and enforces sparsity within each expert.}
    \label{fig:enter-label}
\end{figure}

A central obstacle to mechanistic interpretability is \emph{polysemanticity}, where individual neurons encode multiple, unrelated concepts~\cite{olah2020zoom}. Specifically, we refer to the hidden neurons from the multi-layer perceptron (MLPs) in Transformers. Such polysemantic neurons lack clear, singular roles, making it difficult to identify disentangled features or factors in neural networks. 

A common strategy to address this issue is to decompose entangled neuron activity into interpretable vectors using post-hoc methods like Sparse Auto-Encoders (SAEs)~\cite{huben2023sparse}. However, these approaches are computationally expensive~\cite{gao2024scaling,lieberum2024gemma}, require additional analysis after training, and often do not explain all the features of the model~\cite{menon2024analyzing}.

Instead, we advocate for designing interpretability \emph{directly} into the model architecture, ensuring competitive performance while discouraging polysemanticity during training. Although some works explore architectural changes for interpretability, they often focus on toy-scale tasks~\cite{pearce2024bilinear,agarwal2021neural,sharkey2023technical,jermyn2022engineering} or sacrifice performance~\cite{elhage2022solu}.


To achieve this \emph{intrinsic interpretability}, we propose to leverage mixture-of-experts (MoE) architectures~\cite{fedus2022switch,shazeer2017outrageously}. MoEs naturally partition computation across multiple specialized experts, potentially leading to intrinsic interpretability. However, standard MoE models still struggle to match the interpretability of post-training SAEs.

To understand this gap, we analyze the key differences between MoE and SAE and identify the factors influencing their interpretability. We make two key observations
\begin{itemize}
    \item The success of SAEs largely depends on increasing the size of MLP layers (i.e., the number of hidden activations) while enforcing sparsity in these activations.
    \item Despite their structural differences, MoEs can be viewed as large, sparse MLPs, where expert neurons are selectively weighted based on sparse gating scores. This suggests that MoEs could inherit the interpretability benefits of SAEs if properly structured.
\end{itemize}


Building on these insights, we propose \textbf{MoE-X}, a modified MoE architecture designed to replicate the interpretability benefits of SAEs. The key distinction is that standard MoEs enforce \emph{structured sparsity}, while SAEs impose fully sparse activations. To ensure full sparsity across all concatenated expert features, MoE-X enforces sparsity within each expert while ensuring the router selects the sparsest experts. This is achieved through two key modifications:

% To address these challenges, MoE-X introduces two key innovations:

\textbf{ReLU Experts.} We use \texttt{ReLU} activation within each expert. This simple yet effective modification promotes intrinsic activation sparsity in the expert~\cite{awasthi2024learning}, which in turn helps to disentangle the feature representations.

\textbf{Sparsity-Aware Routing.} We introduce a gating function that predicts which experts would produce the most sparse activations. To avoid expensive computations, we develop a method to estimate each expert’s sparsity \emph{without} explicitly computing all activations. This ensures that the sparsest experts are chosen during inference, promoting disentangled representations.

Together, these modifications enable MoE-X to maintain competitive performance while providing more transparent, semantically meaningful internal representations.Our experiments on chess and language tasks confirm that MoE-X matches or exceeds the performance of dense Transformers while eliminating the need for expensive post-hoc interpretability methods.
% By making mild assumptions on the weight distributions, we derive a closed-form estimate of each 
% \bibi{I do not think this is all very necessary; you could just say that we procide a crude theoretical justification behind such a choice}
% expert’s sparsity and route inputs accordingly,  \emph{without} having to compute the activations of all experts explicitly.




% (1) the sucess of SAE largely relied on the increasing the size of the MLP layers, i.e., number of hidden activations, and the sparsity of these activations. (2) While looks different, MoE can be rewritten as a wide and sparse MLP, similar to SAE.  neurons are weighted by the sparse gating scores.  single bigger MLP layer



% Motivated by these findings, we propose MoE-X, a modified MoE architecture that resemble the success of SAE in interpretability. the rewrited large MLP from MoE is \emph{structued sparse}. enforce sparsity across this whole vector concatenated expert features. First, each expert is still a dense MLP, which can suffer from polysemanticity. Second, standard \emph{top-k} routing~\cite{fedus2022switch} primarily targets performance rather than expert sparsity. As a result, the gating decisions made by the routing mechanism are often misaligned with the goals of interpretability. 


% To bridge this gap and align MoE with interpretability, we propose \textbf{MoE-X}, which includes two key designs:



% This structure makes MoE a good candidate to increase the width while maintaining controlled sparsity, leading to inherently interpretable models.


% That is to say, making the MLP layers in a transformer architecture \emph{wider} and \emph{sparser} should encourage more disentangled internal representations. To test this beyond toy experiments~\cite{jermyn2022engineering,elhage2022superposition}, we conduct experiments on GPT-2-like~\cite{radford2019language} models on chess gameplay data~\cite{karvonen2024measuring}. Chess provides an excellent natural ``ground truth'' for interpretability because the board state can be used as a reference for understanding how each neuron represents and predicts chess moves. Our experiments show that a sufficiently wide-and-sparse MLP in transformer indeed yields more interpretable neurons, leading to a 25\% increase in F1 score for chess move prediction, supporting our hypothesis.

% Motivated by these findings, we propose to leverage mixture-of-experts (MoE) architectures~\cite{fedus2022switch,shazeer2017outrageously} as a natural fit for \emph{intrinsic interpretability}. While different from a standard MLP, MoE can be rewritten as a wide and sparse MLP, whose neurons are weighted by the sparse gating scores. This structure makes MoE a good candidate to increase the width while maintaining controlled sparsity, leading to inherently interpretable models.

% +{This gives us a way at which we can change certain "parameters" in the MoE such that the archticture is now equivalent to a transformer architecture where we can now increase the "widness" through archtiectural change and the "sprasity" through regulations to inherently end up with intrinsiclaly interpretable models.}

% By rewriting the MoE layer, we show that it can be regarded as a large, sparse MLP. This aligns with the widely held belief in mechanistic interpretability that \emph{wider} and \emph{sparser} layers foster more distinct feature representations~\cite{elhage2022superposition}.



% Yet, typical MoE models are not optimized for interpretability. \bibir{I think you want to move this much earlire. after you say that MLP layers that are wider and with sparser activations are more interpretable and that you are looking for an inherently interpretable model. Say, a natural choice for an inherently interpretable models are the MoEs (cite). However, they have not been competitive with expensive post training methods like SAE. [here then talk about this observation of these two factors (widness + sparsity and how you show a rewrite allowing you to control MoEs to be more itnerpratable and make and then give your intuition behind this connection/rewrite]}



% \bibir{here you want to link your two changes back to the two key factors you observed. maybe have two bullet points one called Widness and one called sparsity. In wideness say that our rewrite of MoE shows that the activations of all experts can be seen as a single bigger MLP layer. the second point is sparsity. here you say how do you enforce sparsity across this whole vector concatenated expert features. say that this is not obvious given that the gating function selects the activations of full vectors (e.g., experts) all at once in which after concatination the resultant activation might not be sparse. to address that we do two changes. >> then speak about sparsity routing and relu}




In summary, our main contributions are:
\begin{enumerate}
    \item We systematically analyze how architectural choices—particularly width and sparsity—influence interpretability in transformer-based language models. 
    \item We introduce MoE-X, a redesigned MoE layer that functions as a wide, sparse, and more interpretable MLP within large language models.
    \item We incorporate \emph{ReLU Experts} and \emph{Sparsity Routing} to tightly connect gating decisions with the expected sparsity of activations.
    \item Our experiments on chess tasks demonstrate that MoE-X models achieve strong performance while offering clear and interpretable representations.
\end{enumerate}



% \bibir{over all okish summary but a few comments regarding the flow of the idea/motivation.
% 1. start by saying in interpretability has been a major challenge in recent years for these big models given the risks associated with deploying them at safe critical applications. 
% 2. This has incited an exiting rich research on mechansitic interpretability, a post training approach towards interprting model decisions, i.e., identifyign which nodes contributed to what decision.
% 3. However, polysemanticity has been a major obstecale as [neurons have mixed concepts ..]
% 3. to address this issue, mech interp people do SAE. which is the most popluar mehtods with impressive performance.
% 4. the issue is that SAEs are a) .. b) .. c) [mention all drawbacks -- post training, expensive, etc etc]
% 5. There is a need towards new architectures that are inherently interpretable with no need for pos training mechanisms, methods that perform well and are interpretable.
% 6. a natural candidate is the MoE family; however, they do not still compete well with post training SAE.
% 7. We make two observations. First, we observe that SAEs with larger number of MLP activation while being sparser are far far better in interpretation. the second observation is that, we can show that MoEs are closely related to SAEs, and in fact, can be written as a special type of SAEs. 8. inspired by this we propose two changes to the MoE architecture [talk about the relus and gating] in which we end up with MOEs that are equivalent to wider and sparse SAEs.
% 9. we traing these new models, we call MoE-X, and show strong evidence that they enjoy impressive interpretability results without scarifying the overall performance, i.e., inherently interpretable. 
% 10. To that end, our contributions can be summarized into 3 folds}



% A common strategy to address this is to decompose these tangled neurons into interpretable vectors. Sparse dictionary learning techniques, such as Sparse Auto-Encoders (SAEs)~\cite{huben2023sparse}, attempt this by identifying sparse directions in activation space. However, they are computationally costly~\cite{gao2024scaling,lieberum2024gemma}, require post-hoc analysis, and often fail to recover all relevant features after the model is trained.

% To close this gap, we advocate for an approach that designs interpretability directly into the model architecture itself, thereby discouraging polysemanticity all from the start. Specifically, we focus on making the hidden activations of MLP layers in Transformers more interpretable. While some methods explore architectures with intrinsic interpretability, they either focus on smaller tasks~\cite{pearce2024bilinear,agarwal2021neural,sharkey2023technical, jermyn2022engineering} or compromise performance~\cite{elhage2022solu}.



% The built-in interpretability eliminates costly post-hoc analysis, providing a practical and faithful pathway to understanding large language models. Specifically, our contributions are:

% To reconcile performance with interpretability, we make two architecture fix. For the first question, we use \texttt{ReLU} expert to make experts intrincially sparsely activated. For the second question, we introduce \textbf{sparse-routing}, which estimate the activation sparsity and selects sparest ones for model inference. By give moderate assumption on the weight distribution, we can estimate the hidden neuron sparsity in close form, without running each expert. As such, we select the experts with largest sparsity, which a more faithful representation of the experts’ contributions and offers greater transparency into the network’s internal decision-making.

% We introduce \textbf{MoE-X}, a redesign of the classic MoE that enhances interpretability.


% First, by rewriting the MoE layer, we show it can be viewed as a large, sparse MLP—fulfilling the widely held belief in mechanistic interpretability that \emph{wider} and \emph{sparser} layers foster more distinct feature representations. We validate this belief using GPT-2-like\cite{radford2019language} models on chess gameplay data (Portable Game Notation), exploiting the chessboard state as a natural interpretability ground truth~\cite{karvonen2024measuring}. 

 % And so the question is, how can we create a neural network architecture which will encourage features to align with neurons, and discourage polysemanticity? This means training models whose internal representations are naturally monosemantic and easy to understand, without the need for additional tools like SAEs.
 % While there are method that aims to looks for intricically interpretable architecture designs, nor do they conpensate performance~\cite{elhage2022solu}, nor they focus on toyish tasks~\cite{pearce2024bilinear,agarwal2021neural,sharkey2023technical, jermyn2022engineering}.


% In this work, we take a radically different approach. Instead of relying on post-hoc interpretability tools, we show that the mixture of expert large language models (LLMs) is natural fit for \textbf{intrinsically interpretable}. Beside that, we redesign a new MoE-X model to even enhance the interp

% To show why this is indeed reasonable, we first verify two common beliefs in mech interp that \textbf{Wide} and \textbf{Sparse} in the full connected layers gives better interp. Specifically, we train GPT-2~\cite{radford2019language} like language model on chess gameplay data represented in Portable Game Notation (PGN) as a language modeling task, we leverage the chessboard state as a natural ground truth for interpretability~\cite{karvonen2024measuring}. By vary the model setup, we see that Wider but sparse transformers exhibit greater interpretability by allowing more distinct feature representations. 


% Those motivation natrually lead to us to MoE architectures, which are born to be Wider and sparse. By a simple rewrite of the MoE inference, we can see a MoE as a MLP with super large but sparse activated neurons~\cite{liu2023towards} composed of original activation values and gating scores, where the activation shows structure sparsity. This modular design supports the disentanglement of features, making it easier to associate specific behaviors or concepts with individual components of the model. It allow us to create language model.

% To investigate this, we focus on the MLP layers in causal transformer-based LLMs and study the factors that govern their interpretability. 
% Using chess gameplay data represented in Portable Game Notation (PGN) as a language modeling task, we leverage the chessboard state as a natural ground truth for interpretability~\cite{karvonen2024measuring}. Our experiments reveal three key factors that significantly influence model interpretability:

% \begin{itemize} 
% \item Model width: Wider transformers exhibit greater interpretability by allowing more distinct feature representations.
% \item Sparsity: Moderately sparse activations strike a balance between feature distinctiveness and efficiency.
% % \item Training duration: Longer training times lead to more refined and semantically meaningful feature representations.
% \end{itemize}

% To realize these principles, we turn to \textbf{Mixture-of-Experts (MoE)} architectures, which naturally align with our interpretability objectives. 

% MoE models partition their capacity into distinct expert modules, enabling scalable increases in representational capacity while preserving sparsity. This modular design supports the disentanglement of features, making it easier to associate specific behaviors or concepts with individual components of the model. By incorporating MoE architectures, we extend the dictionary learning framework to a scalable and interpretable regime, where each concept is mapped to a sparsely activated dictionary atom.
